Orchestral AI: A Framework for Agent Orchestration

The rapid proliferation of LLM agent frameworks has forced developers to choose between vendor lock-in through provider-specific SDKs and complex multi-package ecosystems that obscure control flow and hinder reproducibility. Integrating tool calling across multiple LLM providers remains a core engineering challenge due to fragmented APIs, incompatible message formats, and inconsistent streaming and tool-calling behavior, making it difficult to build portable, reliable agent systems. We introduce Orchestral, a lightweight Python framework that provides a unified, type-safe interface for building LLM agents across major providers while preserving the simplicity required for scientific computing and production deployment. Orchestral defines a single universal representation for messages, tools, and LLM usage that operates seamlessly across providers, eliminating manual format translation and reducing framework-induced complexity. Automatic tool schema generation from Python type hints removes the need for handwritten descriptors while maintaining type safety across provider boundaries. A synchronous execution model with streaming support enables deterministic behavior, straightforward debugging, and real-time interaction without introducing server dependencies. The framework's modular architecture cleanly separates provider integration, tool execution, conversation orchestration, and user-facing interfaces, enabling extensibility without architectural entanglement. Orchestral supports advanced agent capabilities found in larger frameworks, including rich tool calling, context compaction, workspace sandboxing, user approval workflows, sub-agents, memory management, and MCP integration.

==> orchestral_whitepaper_arxiv_v1/orchestral.tex <==
% Orchestral LaTeX Module - MINIMAL VERSION
% Only the essential definitions needed for the paper

% Suppress tcolorbox tagging output by redefining commands BEFORE tcolorbox loads
\makeatletter

% Swallow all tagging-related commands that produce visible output
\def\NewStructureName#1{}
\def\AssignStructureRole#1#2{}
\def\NewTaggingSocket#1#2{}
\def\NewTaggingSocketPlug#1#2#3{}
\def\AssignTaggingSocketPlug#1#2{}
\def\UseStructureName#1{}
\def\tagstructbegin#1{}
\def\tagstructend{}
\def\tagpdfparaOff{}

\makeatother

\usepackage{tcolorbox}
\tcbuselibrary{skins,breakable}

% Color Definitions
\definecolor{OrcUserColor}{RGB}{60, 60, 60}
\definecolor{OrcAgentColor}{RGB}{120, 120, 255}
\definecolor{OrcToolColor}{RGB}{200, 100, 0}
\definecolor{OrcFailedColor}{RGB}{220, 20, 60}

% User message box
\newtcolorbox{orchestralusermessage}{
  enhanced,
  breakable,
  colback=white,
  colframe=OrcUserColor,
  boxrule=0.6pt,
  arc=1.5mm,
  width=\linewidth,
  top=8pt,
  bottom=8pt,
  left=10pt,
  right=10pt,
  fontupper=\small,
  attach boxed title to top left={yshift=-6pt, xshift=3.5mm},
  boxed title style={colback=white, colframe=white, boxrule=0pt},
  coltitle=OrcUserColor,
  fonttitle=\sffamily,
  title={\raisebox{0pt}[0pt][0pt]{User}},
}

% Agent message box
\newtcolorbox{orchestralagentmessage}{
  enhanced,
  breakable,
  colback=white,
  colframe=OrcAgentColor,
  boxrule=0.6pt,
  arc=1.5mm,
  width=\linewidth,
  top=8pt,
  bottom=8pt,
  left=10pt,
  right=10pt,
  fontupper=\small,
  attach boxed title to top left={yshift=-6pt, xshift=3.5mm},
  boxed title style={colback=white, colframe=white, boxrule=0pt},
  coltitle=OrcAgentColor,
  fonttitle=\sffamily,
  title={\raisebox{0pt}[0pt][0pt]{Agent}},
}

% Tool message box (takes one argument: tool title)
\newtcolorbox{orchestraltoolmessage}[1]{
  enhanced,
  breakable,
  colback=white,
  colframe=OrcToolColor,
  boxrule=0.5pt,
  arc=1mm,
  width=\linewidth,
  left=1.5em,
  right=1em,
  top=6pt,
  bottom=6pt,
  fontupper=\small,
  attach boxed title to top left={yshift=-5pt, xshift=3.5mm},
  boxed title style={colback=white, colframe=white, boxrule=0pt},
  coltitle=OrcToolColor,
  fonttitle=\sffamily\small,
  title={\raisebox{0pt}[0pt][0pt]{#1}},
}

% Tool error message box (takes one argument: tool title)
\newtcolorbox{orchestraltoolerrormessage}[1]{
  enhanced,
  breakable,
  colback=white,
  colframe=OrcFailedColor,
  boxrule=0.6pt,
  arc=1mm,
  width=\linewidth,
  left=1.5em,
  right=1em,
  top=6pt,
  bottom=6pt,
  fontupper=\small,
  attach boxed title to top left={yshift=-5pt, xshift=3.5mm},
  boxed title style={colback=white, colframe=white, boxrule=0pt},
  coltitle=OrcFailedColor,
  fonttitle=\sffamily\small,
  title={\raisebox{0pt}[0pt][0pt]{#1}},
}

